ReFineVLA: Multimodal Reasoning-Aware Generalist Robotic Policies via Teacher-Guided Fine-Tuning

Vision-Language-Action (VLA) models have gained much attention from the research community thanks to their strength in translating multimodal observations with linguistic instructions into desired robotic actions. Despite their advancements, VLAs often overlook explicit reasoning and learn the functional input-action mappings, omitting crucial logical steps, which are especially pronounced in interpretability and generalization for complex, long-horizon manipulation tasks. In this work, we propose ReFineVLA, a multimodal reasoning-aware framework that fine-tunes VLAs with teacher-guided reasons. We first augment robotic datasets with reasoning rationales generated by an expert teacher model, guiding VLA models to learn to reason about their actions. Then, we fine-tune pre-trained VLAs with the reasoning-enriched datasets with ReFineVLA, while maintaining the underlying generalization abilities and boosting reasoning capabilities. We also conduct attention map visualization to analyze the alignment among visual observation, linguistic prompts, and to-be-executed actions of ReFineVLA, reflecting the model is ability to focus on relevant tasks and actions. Through this additional step, we explore that ReFineVLA-trained models exhibit a meaningful agreement between vision-language and action domains, highlighting the enhanced multimodal understanding and generalization. Evaluated across a suite of simulated manipulation benchmarks on SimplerEnv with both WidowX and Google Robot tasks, ReFineVLA achieves state-of-the-art performance, in success rate over the second-best method on the both the WidowX benchmark and Google Robot Tasks.

==> tables/full_fractal_googlerobot_table2.tex <==
\begin{table*}[h]
    \centering
    \caption{\textbf{Evaluated performances of different VLA baselines on SimplerEnv with Google Robot tasks:} The zero-shot and fine-tuning results denote the performance of the pre-traineđ models on the OXE dataset \citep{o2024open} and the fine-tuned models on the Fractal dataset \citep{brohan2022rt}, respectively.}
    \label{tab:simplerenv_google_robot} 
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{r cccc cccc}
        \toprule 
        \multirow{3}{*}{\diagbox{VLA Baseline}{Robotic Task}} & \multicolumn{4}{c}{\makecell{\textbf{Visual Matching}}} & \multicolumn{4}{c}{\makecell{\textbf{Variant Aggregation}}} \\
        \cmidrule(lr){2-9}
        & \makecell{Pick \\Coke Can} & Move Near & \makecell{Open/Close \\Drawer} & Average & \makecell{Pick \\Coke Can} & Move Near & \makecell{Open/Close \\Drawer} & Average \\
        \midrule \midrule 
        RT-1 (begin) \citep{brohan2022rt} & 2.7\% & 5.0\% & 13.9\% & 6.8\%  & 2.2\% & 4.0\% & 6.9\% & 4.2\% \\
        RT-1 ($15\%$) \citep{brohan2022rt} & 71.0\% & 35.4\% & 56.5\% & 60.2\% & 81.3\% & 44.6\% & 26.7\% & 56.2\% \\
        RT-1 (converged) \citep{brohan2022rt} & 85.7\% & 44.2\% & 73.0\% & 74.6\% & 89.8\% & 50.0\% & 32.3\% & 63.3\% \\
        \midrule 
        HPT \citep{wang2024scaling} & 56.0\% & 60.0\% & 24.0\% & 46.0\% & -- & -- & -- & -- \\
        TraceVLA \citep{zheng2024tracevla} & 28.0\% & 53.7\% & 57.0\% & 42.0\% & 60.0\% & 56.4\% & 31.0\% & 45.0\% \\
        RT-1-X \citep{o2024open} & 56.7\% & 31.7\% & 59.7\% & 53.4\% & 49.0\% & 32.3\% & 29.4\% & 39.6\% \\
        RT-2-X \citep{o2024open} & \textbf{78.7\%} & 77.9\% & 25.0\% & 60.7\% & 82.3\% & 79.2\% & 35.3\% & 64.3\% \\
        Octo-Base \citep{team2024octo} & 17.0\% & 4.2\% & 22.7\% & 16.8\% & 0.6\% & 3.1\% & 1.1\% & 1.1\% \\
        OpenVLA \citep{kim2024openvla} & 16.3\% & 46.2\% & 35.6\% & 27.7\% & 54.5\% & 47.7\% & 17.7\% & 39.8\% \\
        \midrule 
        RoboVLM (zero-shot) \citep{li2024towards} & 72.7\% & 66.3\% & 26.8\% & 56.3\% & 68.3\% & 56.0\% & 8.5\% & 46.3\% \\
        RoboVLM (fine-tuning) \citep{li2024towards} & 77.3\% & 61.7\% & 43.5\% & 63.4\% & 75.6\% & 60.0\% & 10.6\% & 51.3\% \\
        \midrule 
        SpatialVLA (zero-shot) \citep{qu2025spatialvla} & 81.0\% & 69.6\% & 59.3 \% & 71.9\% & 89.5\% & 71.7\% & 36.2\% & 68.8\% \\
        SpatialVLA (fine-tuning) \citep{qu2025spatialvla} & 86.0\% & \textbf{77.9\%} & 57.4\% & \textbf{75.1\%} & 88.0\% & 72.7\% & 41.8\% & 70.7\% \\
        \midrule
        \rowcolor{gray!15} \textbf{\textit{ReFineVLA} (Ours)} & 74.3\% & 75.0\% & \textbf{62.5}\% & 70.6\% & \textbf{91.6}\% & \textbf{93.2}\% & \textbf{43.2}\% & \textbf{76.0}\% \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-5pt}
\end{table*}
